Adaptive nonparametric drift estimation for diffusion processes using Faber-Schauder expansions

We consider the problem of nonparametric estimation of the drift of a continuously observed one-dimensional diffusion with periodic drift. Motivated by computational considerations, van der Meulen e.a. (2014) defined a prior on the drift as a randomly truncated and randomly scaled Faber-Schauder series expansion with Gaussian coefficients. We study the behaviour of the posterior obtained from the prior from a frequentist asymptotic point of view. If the true data generating drift is smooth, it is proved that the posterior is adaptive with posterior contraction rates for the $L_2$-norm that are optimal up to a log factor. Moreover, contraction rates in $L_p$-norms with $p\in (2,\infty]$ are derived as well.

==> math0.tex <==

\makeatletter
\newcommand*{\DeclareMathOperators}[1]{%
	\@for\@tmp:=#1\do{%
		% remove spaces
		\edef\@tmp{%
			\@firstofone{\expandafter\zap@space\@tmp} \@empty
		}%
		\ifx\@tmp\@empty
		\else
		% declare math operator
		\expandafter\DeclareMathOperator
		\csname\@tmp\expandafter\endcsname\expandafter{\@tmp}%
		% \wlog prints into the .log file
		% or \typeout can be used for console output                      
		\wlog{* Math operator "\@backslashchar \@tmp" defined.}%
		\fi
	}%
}
\makeatother

\newcommand{\si}{\sigma}
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\th}{\theta}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\ka}{\kappa}
\newcommand{\weg}{\backslash}

\newcommand{\legeregel}{\par\vspace{1ex}\noindent}
\newcommand{\isd}{\stackrel{d}{=}}
\newcommand\Sgn{\mathop{\mathrm{Sgn}}\nolimits}
\newcommand\Log{\mathop{\mathrm{Log}}\nolimits}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\nphi}{\phi}
\renewcommand{\phi}{\varphi}
\newcommand{\asnaar}{\stackrel{\mathrm{a.s.}}{\longrightarrow}}
\newcommand{\pto}{\stackrel{\mathrm{p}}{\longrightarrow}}
%\newcommand{\wto}{\stackrel{\mathrm{w}}{\longrightarrow}}
\newcommand{\wto}{\rightsquigarrow}
\newcommand{\asto}{\stackrel{\mathrm{a.s.}}{\longrightarrow}}
\newcommand{\dto}{\stackrel{\mathrm{\scr{D}}}{\longrightarrow}}
\newcommand{\scr}[1]{{\mathcal #1}}
\newcommand{\mf}[1]{{\mathfrak #1}}  %package eufrak required
\newcommand{\ms}[1]{{\mathscr #1}}  %package eufrak required

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
%\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\TT}{\mathbb{T}}
\DeclareMathOperator{\T}{\mathbb{T}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\DeclareMathOperator{\N}{\mathbb{N}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\renewcommand{\vec}[1]{\underline{ #1}}
\newcommand{\Ell}{\mathcal{L}}


\newcommand{\mb}[1]{\mathbf{ #1}}
\newcommand{\ft}[1]{\frametitle{#1}}

\newcommand{\bem}{\begin{bmatrix}}
\newcommand{\enm}{\end{bmatrix}}

%\newcommand{\cit}{\citeNP}
\newcommand{\as}{\ensuremath{\text{a.s.}}}
\newcommand{\Pas}[1]{\ensuremath{#1\text{-a.s.}}}

\newcommand{\e}{\mathrm{e}}

\renewcommand{\P}{\ensuremath{{\mathrm P}}}
\newcommand{\Q}{\ensuremath{{\mathrm Q}}}
\newcommand{\dP}{\ensuremath{{\mathrm d \mathrm P}}}
\newcommand{\dQ}{\ensuremath{{\mathrm d\mathrm Q}}}


\newcommand{\prob}[1]{\ensuremath{{\mathrm P}\!\left( #1 \right)}}
\newcommand{\prc}[2]{\ensuremath{{\mathrm P}( #1 \, |\, #2)}}
\newcommand{\expec}[1]{\ensuremath{{\mathrm E}\mspace{-1mu}\left[#1\right]}}
%\newcommand{\cexpec}[2]{\ensuremath{{\mathrm E}\mspace{-1mu}\left[#1\big|#2\right]}}

\newcommand{\E}{\mathrm{E}\,}
\newcommand{\var}[1]{\ensuremath{{\mathrm Var}\!\left( #1 \right)}}
\newcommand{\cov}[2]{\ensuremath{{\mathrm Cov}\!\left( #1 , #2 \right)}}
%\newcommand{\cor}[2]{\ensuremath{{\rho}\mspace{-1mu}\left( #1 , #2 \right)}}
\newcommand{\mean}[1]{\ensuremath{\bar{#1}}}
\newcommand{\Id}{\mathrm I}
\newcommand{\ind}{{\mathbf{1}}}
\opt{bbm}{
\renewcommand{\ind}{{\mathbbm{1}}}
}
\opt{bbold}{
\renewcommand{\ind}{\mathbbold{1}}
}
\newcommand{\pin}[1]{{#1}^\star}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\DD}{{\,\mathrm D}}
\newcommand{\dd}{{\,\mathrm d}}
\providecommand{\I}{\mathrm{I}}
 
\newcommand{\dprime}{{\prime\prime}}
%\newcommand{\dhp}{{\circ\!\text{'}}}
%\newcommand{\mbb}{{\circ\!\text{''}}}
\newcommand{\dhp}{{\!\triangledown}}
\newcommand{\mbb}{{\!\vartriangle}}
%\newcommand{\mbb}{{\circ\!\text{''}}}
\newcommand{\gpp}{{\tilde{\circ}}}
\newcommand{\qv}[1]{\left<{#1}\right>}

\newcommand{\thmnewline}{\mbox{}
\vspace*{-\parsep}%
%\vspace*{-\baselineskip}
}
%finally a colvec
\newcount\colveccount
\newcommand*\colvec[1]{
        \global\colveccount#1
        \begin{pmatrix}
        \colvecnext
}
\def\colvecnext#1{
        #1
        \global\advance\colveccount-1
        \ifnum\colveccount>0
                \\
                \expandafter\colvecnext
        \else
                \end{pmatrix}
        \fi
}


 



\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}


\newcommand{\linecont}{\hspace{0.1\textwidth}}


\newcommand{\qtext}[1]{\quad\text{#1}\quad}
